Transfer Learning for Input Estimation of Vehicle Systems

This study proposes a learning-based method with domain adaptability for input estimation of vehicle suspension systems. In a crowdsensing setting for bridge health monitoring, vehicles carry sensors to collect samples of the bridge's dynamic response. The primary challenge is in preprocessing; signals are highly contaminated from road profile roughness and vehicle suspension dynamics. Additionally, signals are collected from a diverse set of vehicles vitiating model-based approaches. In our data-driven approach, two autoencoders for the cabin signal and the tire-level signal are constrained to force the separation of the tire-level input from the suspension system in the latent state representation. From the extracted features, we estimate the tire-level signal and determine the vehicle class with high accuracy (98% classification accuracy). Compared to existing solutions for the vehicle suspension deconvolution problem, we show that the proposed methodology is robust to vehicle dynamic variations and suspension system nonlinearity.

==> 0A_Extra.tex <==
ICASSP 2021
https://2021.ieeeicassp.org/
https://2021.ieeeicassp.org/Papers/PaperKit.asp

Future things:
1) Separate VLF from road
    - System prop estimations
    - If road and suspension are actually separate... can you substitute?
    - maybe try VAE as well
2) Train R-AE. Freeze weights. Train V-AE.
3) Try to disjoint the method completely by making the RLF more flexible 4) SM and USM unsupervised separating RLF
4) Maybe instead of cherry picking create a boundary in frequency that is reliable.

Topics: 15.4.2*:	Autonomous and Cyber-Physical Systems

==> Response_Letter.tex <==
We would like to take this opportunity, and thank the referees for taking the time to review our work and are grateful for their insightful comments. The response contains references from the referees' comments and the manuscript's changes to address it when required.

1. We address comments by referees (05B5, 19AF) regarding the numerical analysis and the use of real data for this study:

Reviewer 05B5: "While I understand the difficulties of working with real data, and the advantages of being able to train on synthetically generated data, it would have been nice to have some real-world data involved."

Reviewer 19AF: "The proposed methodology is very complex with lots of potential sources of error. The results provided by the paper are also partial, not yet confirming if the proposed approach is fully implementable in the proposed way."

We acknowledge the fact that the application of the proposed network was shown for a numerical example. However, it is important to note that the problem of vehicle suspension deconvolution is a complex yet useful problem that has been rarely studied previously. In particular, the approach taken in this study enables extracting insights regarding vehicle and road types, which is unique. Therefore, we consider this study as a pilot work and use numerical examples as a proof of concept. In the next step, we will conduct a full-scale experiment that will consider a variety of new aspects to this problem, which we deemed outside this initial study's scope, such as sensor location and orientation, signal-noise ratio, road profile nonstationarity, vehicle dynamical dependence to temporal changes, etc. 

2. Reviewer 05B5 was also concerned with the 1% variation on system parameters. 

Reviewer 05B5: "Also, the 1% variations of the parameters that were used to test the robustness of the system are somewhat optimistic in terms of the tolerances in vehicular manufacture."

We agree that this may be optimistic. For this reason, we repeated our analysis with 5%, 10%, 15%, 20%, 30% and 40% variations. We found the following classification accuracy percentages for these cases: 92.8%, 91.2%, 85.6%, 87.2%, 76.%, and 67.8%, respectively. In the revised manuscript, we will update Figure 4 and the associated text. 

3. Reviewer 1EC1 noted a lack of review and comparison to a more classical signal processing approach such as digital adaptive filtering (DAF):

Reviewer 1EC1: "This paper addresses the issue of extracting high-level information from noisy sensory signals. The transfer learning based technique proposed with two autoencoders are utilized to separate the road latent feature (RLF) and vehicle latent feature (VLF) from the original cabin signal. The major issue of the paper is lack of sufficient comparisons over conventional techniques such as digital adaptive filtering."

In response, we would like to emphasize on multiple aspects of the proposed method that cannot be replicated by using classical filtering methods. a) the proposed method is not a model-based solution as opposed to the large group of DAFs, b) the method shows efficacy in learning nonlinearities with no prior information about the underlying function, and c) the method provides insights regarding the vehicle and the road as byproducts of the main algorithm. Overall, we agree that a comparison with classical methods will benefit the paper. However, due to the space limitations, this will be reserved for a more extensive study. 

4. Reviewer 05B5 was concerned about using the term transfer function as the system we describe is nonlinear:

Reviewer 05B5: "One technical issue that arises in the experiment section is the use of the term "transfer function". Transfer functions are a great analysis tool for linear systems, but the authors have just explained the importance of including non-linearities in their system model. As a result, it is a little hard to understand what the authors are doing here. Is this the transfer function of the linear component of a Volterra series model? Is it the transfer function of the linearized model at low speeds, or the linearized model at high positive or negative speeds? (see Fig 3)"

We agree with the reviewer's concern on the use of the term "transfer function" for nonlinear dynamic systems. The input-output relationship for a nonlinear dynamic system will be a function of both frequency and input amplitude unlike transfer functions in linear systems. The functions shown in figure 5 of the manuscript were derived by averaging the input-output relationship for a range of input impulse amplitudes. This was done for easily visualizing the input-output relationship for interpreting the performance of the proposed framework. 

With regards to a scientifically accurate terminology, in the nonlinear dynamics research community, we have come across works that take recourse to approximations referred to as "effective transfer functions" and "describing functions" wherein the dependence on the input amplitude is addressed and approximate functions akin to traditional transfer functions are developed. To address the ambiguity with regards to the terminology, in the revised manuscript we will update the caption of figure 5 and the associated text with the phrase "nonlinear transfer function" and its clear definition. 
